On the Ergodic Secrecy Capacity of Reconfigurable Intelligent Surface Aided Wireless Systems Under Mixture Gamma Fading

This paper presents a quantified assessment of the physical layer security capabilities of reconfigurable intelligent surface (RIS)-aided wireless systems under eavesdropping. Specifically, we derive a closed-form expression for the ergodic secrecy capacity (ESC) that is adaptable to different types of fading and RIS size. The channels between the transmitter (TX) and RIS, the RIS and legitimate receiver as well as the TX and eavesdropper are assumed to follow independent mixture Gamma (MG) distributions. Note that MG is capable of modeling a large variety of well-known distributions, including Gaussian, Rayleigh, Nakagami-m, Rice, and others. The results reveal that as the RIS size increases, although the legitimate links diversity order increases, the ESC gain decreases.

==> images/plot1.tex <==
\begin{tikzpicture}
	\begin{axis}[
		xlabel={$\beta_B^{2}\,\mathrm{(dB)}$},
		ylabel={$C_s\,\mathrm{(bits/s/Hz)}$},
		legend pos=north west,
		xmin = 0,
		xmax =1,
		ymin = 0,
		ymax= 0.5,
	%	xtick = {-30,  -20,  -10,  0, 10, 20},
	%	ytick = {0, 2, 4, 6, 8, 10, 12, 14, 16},
		ymajorgrids=true,
		xmajorgrids=true,
		grid style=dashed,
		]
		
		\addplot[dashed,
		color=black]
		coordinates {
			(0, 0.368678)
			(0.01, 0.368678)
			
		};
	\addlegendentry{\small{Analytical (N=8)}}
	
\end{axis}

\end{tikzpicture}
